Combining Combination Properties: Minimal Models

This is a part of an ongoing research project, with the aim of finding the connections between properties related to theory combination in Satisfiability Modulo Theories. In previous work, 7 properties were analyzed: convexity, stable infiniteness, smoothness, finite witnessability, strong finite witnessability, the finite model property, and stable finiteness. The first two properties are related to Nelson-Oppen combination, the third and fourth to polite combination, the fifth to strong politeness, and the last two to shininess. However, the remaining key property of shiny theories, namely, the ability to compute the cardinalities of minimal models, was not yet analyzed. In this paper we study this property and its connection to the others.

==> Table.tex <==
\afterpage{
\crefname{theorem}{theorem}{theorems}
\Crefname{theorem}{Theo.}{Theo.}

\renewcommand{\arraystretch}{1.0}
\begin{longtable}{|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}||P{1cm}P{1cm}P{1cm}P{1cm}|P{0.5cm}|}
%[htp]
%\setlength{\tabcolsep}{1pt}
%\centering
%\begin{tabular}
\hline
\multicolumn{8}{|c|}{} & \multicolumn{2}{c|}{Empty} & \multicolumn{2}{c|}{Non-empty} & \\
\hline
$\stainf$ & $\smooth$ & $\finwit$ & $\strfinwit$ & $\convex$ & $\finmodpro$ & $\stafin$ & $\cmmf$ & \multicolumn{1}{c|}{OS} & \multicolumn{1}{c|}{MS} &\multicolumn{1}{c|}{OS} & \multicolumn{1}{c|}{MS}& $N^{\underline{o}}$\\\hhline{-------------}

\multirow{36}{*}{$T$ } & \multirow{20}{*}{$T$ } &
\multirow{12}{*}{$T$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
1\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\Cref{SM+ES=>CMMF}\cellcolor{red!15}}&
\multicolumn{2}{c|}{\textcolor{red}{Unicorns 2.0}}&
2\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{2}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
3\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-2}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{2}{c|}{\textcolor{red}{Unicorns 2.0}}&
4\\\hhline{~~~----------}

 &  &
 & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{2}{c|}{\textcolor{red}{Unicorns 3.0}}&
5\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}} &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
6\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
7\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{\Cref{SM+ES=>CMMF}\cellcolor{red!15}}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
8\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{2}{c|}{\textcolor{red}{Unicorns 3.0}}&
9\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
10\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
11\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|---}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-4}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
12\\\hhline{~~-----------}

 &  &
\multirow{8}{*}{$F$ } & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
13\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-2}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
14\\\hhline{~~~~~--------}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } & 
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
15\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\Cref{SM+ES=>CMMF}\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
16\\\hhline{~~~~~--------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{2}{*}{$T$ } & 
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
17\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  & 
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
18\\\hhline{~~~~~---*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } & 
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
19\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-4}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
20\\\hhline{~------------}

 & \multirow{16}{*}{$F$ } &
\multirow{8}{*}{$T$ } & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{4}{*}{$T$ } & 
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
21\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
22\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  & 
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
23\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
24\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{4}{*}{$T$ } & 
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
25\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
26\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  & 
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
27\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|---}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-4}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
28\\\hhline{~~-----------}

 &  &
\multirow{8}{*}{$F$ } & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
29\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
30\\\hhline{~~~~~--------}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
31\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\Cref{-FMP+ES+OS=>CMMF}\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
32\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
33\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
34\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
35\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-4}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
36\\\hhline{-------------}

\multirow{20}{*}{$F$ } & \multirow{20}{*}{$F$ } &
\multirow{12}{*}{$T$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
37\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\Cref{-SI+ES=>CMMF}\cellcolor{red!15}}&\multicolumn{3}{c|}{\textcolor{red}{Unicorns 2.0}}&
38\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{2}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
39\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\Cref{-SI+ES=>CMMF}\cellcolor{red!15}}&\multicolumn{3}{c|}{\textcolor{red}{Unicorns 2.0}}&
40\\\hhline{~~~----------}

 &  &
 & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
41\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{CADE}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
42\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
43\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
44\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
45\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\Cref{-SI+ES=>CMMF}\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
46\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
47\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
48\\\hhline{~~-----------}

 &  &
\multirow{8}{*}{$F$ } & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
49\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
50\\\hhline{~~~~~---*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
51\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
52\\\hhline{~~~~----*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
53\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
54\\\hhline{~~~~~---*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
55\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-8}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{}&
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&
56\\\hhline{-------------}

%\end{tabular}
%\vspace{2em}
\caption[Caption for LOF]{Table of possible and impossible cobinations}
\label{tab-summary}
\end{longtable}

\renewcommand{\arraystretch}{1}

\crefname{theorem}{theorem}{theorems}
\Crefname{theorem}{Theorem}{Theorems}}




We now offer a summarized presentation of the results in this paper in \Cref{tab-summary}. To the left of this table one finds columns for each of the model-theoretic properties considered, and whether they are present ($T$, for true) or absent ($F$, for false) in each row: $\stainf$ (stably infinite), $\smooth$ (smooth), $\finwit$ (finitely witnessable), $\strfinwit$ (strongly finitely witnessable), $\convex$ (convex), $\finmodpro$ (finite model property), $\stafin$ (stably finite), and $\cmmf$ (computability of the minimal model function; when a certain combination, and therefore its accompanying row, is missing, that means that combination is not possible. To the right the cells are either blank, meaning there is a theory corresponding to that combination, or shaded red, when the combination is not possible (at least for signatures with finitely many sorts), and are divided in between $4$ columns, corresponding to signatures that are empty or not, and signatures that are one-sorted (OS) or not (MS, standing for many-sorted).

Shaded cells also carry either the result proving that such a combination is impossible, or the reference, among \cite{CADE,FroCoS} that carries such result. The exceptions to the division of cells to the right between blank and shaded cells are those with an updated unicorn theory in it. To explain that, let us circle back to \cite{CADE}: in that paper we could not find theories that were stably infinite and strongly finitely witnessable, but not smooth, and neither could we prove they do not exist; given their elusive nature, and the fact we conjectured they did not exist, we nicknamed them \emph{unicorn theories}.

% Later, in \cite{LICS}, we proved they indeed do not exist, but were forced to use much more abstract tools in model theory: noticed that, because of this, several lines in the table were removed when compared to \cite{CADE,FroCoS}. 















% TABLE BROKEN IN HALF

\afterpage{
\renewcommand{\arraystretch}{0.84}
\begin{longtable}{|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}|P{0.5cm}||P{1cm}P{1cm}P{1cm}P{1cm}|P{0.5cm}|}
%[htp]
%\setlength{\tabcolsep}{1pt}
%\centering
%\begin{tabular}
\hline
\multicolumn{8}{|c|}{} & \multicolumn{2}{c|}{Empty} & \multicolumn{2}{c|}{Non-empty} & \\
\hline
$\stainf$ & $\smooth$ & $\finwit$ & $\strfinwit$ & $\convex$ & $\finmodpro$ & $\stafin$ & $\cmmf$ & \multicolumn{1}{c|}{OS} & \multicolumn{1}{c|}{MS} &\multicolumn{1}{c|}{OS} & \multicolumn{1}{c|}{MS}& $N^{\underline{o}}$\\\hhline{-------------}

\multirow{36}{*}{$T$ } & \multirow{20}{*}{$T$ } &
\multirow{12}{*}{$T$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{$\Tgeqn$}&\multicolumn{1}{c|}{$\adds{\Tgeqn}$}&
\multicolumn{1}{c|}{$\addf{\Tgeqn}$}&\multicolumn{1}{c|}{$\addf{\adds{\Tgeqn}}$}&
1\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\Cref{SM+ES=>CMMF}\cellcolor{red!15}}&
\multicolumn{2}{c|}{\textcolor{red}{Unicorns 2.0}}&
2\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{2}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\addnc{\Tgeqn}$}&\multicolumn{1}{c|}{$\addnc{\adds{\Tgeqn}}$}&
3\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-2}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{2}{c|}{\textcolor{red}{Unicorns 2.0}}&
4\\\hhline{~~~----------}

 &  &
 & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{2}{c|}{\textcolor{red}{Unicorns 3.0}}&
5\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}} &
\multicolumn{1}{c|}{$\TM$}&\multicolumn{1}{c|}{$\adds{\TM}$}&
6\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Ttwothree$}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\addf{\Ttwothree}$}&
7\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{\Cref{SM+ES=>CMMF}\cellcolor{red!15}}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{$\Tseventeen$}&
8\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{2}{c|}{\textcolor{red}{Unicorns 3.0}}&
9\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\TsM$}&\multicolumn{1}{c|}{$\adds{\TsM}$}&
10\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\addnc{\Ttwothree}$}&
11\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|---}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-4}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{$\Teighteen$}&
12\\\hhline{~~-----------}

 &  &
\multirow{8}{*}{$F$ } & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\Tbbs$}&\multicolumn{1}{c|}{$\Tbbeq$}&
13\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-2}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tbbtwo$}&
14\\\hhline{~~~~~--------}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } & 
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{$\Tinfty$}&\multicolumn{1}{c|}{$\adds{\Tinfty}$}&
\multicolumn{1}{c|}{$\addf{\Tinfty}$}&\multicolumn{1}{c|}{$\addf{\adds{\Tinfty}}$}&
15\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\Cref{SM+ES=>CMMF}\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\Tfifteen$}&\multicolumn{1}{c|}{$\adds{\Tfifteen}$}&
16\\\hhline{~~~~~--------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{2}{*}{$T$ } & 
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\Tbbvee$}&\multicolumn{1}{c|}{$\adds{\Tbbvee}$}&
17\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  & 
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tbbveeeq$}&
18\\\hhline{~~~~~---*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } & 
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\addnc{\Tinfty}$}&\multicolumn{1}{c|}{$\addnc{\adds{\Tinfty}}$}&
19\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-4}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{$\Tsixteen$}&\multicolumn{1}{c|}{$\adds{\Tsixteen}$}&
20\\\hhline{~------------}

 & \multirow{16}{*}{$F$ } &
\multirow{8}{*}{$T$ } & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{4}{*}{$T$ } & 
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{$\Teven$}&\multicolumn{1}{c|}{$\adds{\Teven}$}&
\multicolumn{1}{c|}{$\addf{\Teven}$}&\multicolumn{1}{c|}{$\addf{\adds{\Teven}}$}&
21\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{$\Tone$}&\multicolumn{1}{c|}{$\adds{\Tone}$}&
\multicolumn{1}{c|}{$\addf{\Tone}$}&\multicolumn{1}{c|}{$\addf{\adds{\Tone}}$}&
22\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  & 
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tupinfty$}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\adds{\Tupinfty}$}&
23\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{$\Ttwo$}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{$\adds{\Ttwo}$}&
24\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{4}{*}{$T$ } & 
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\addnc{\Teven}$}&\multicolumn{1}{c|}{$\addnc{\adds{\Teven}}$}&
25\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\addnc{\Tone}$}&\multicolumn{1}{c|}{$\addnc{\adds{\Tone}}$}&
26\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  & 
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\addnc{\Tupinfty}$}&
27\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|---}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  & 
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-4}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{$\addnc{\Ttwo}$}&
28\\\hhline{~~-----------}

 &  &
\multirow{8}{*}{$F$ } & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{$\Tbb$}&\multicolumn{1}{c|}{$\adds{\Tbb}$}&
\multicolumn{1}{c|}{$\addf{\Tbb}$}&\multicolumn{1}{c|}{$\addf{\adds{\Tbb}}$}&
29\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tbbinfty$}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\addf{\Tbbinfty}$}&
30\\\hhline{~~~~~--------}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{$\Tninfty$}&\multicolumn{1}{c|}{$\adds{\Tinfty}$}&
\multicolumn{1}{c|}{$\addf{\Tninfty}$}&\multicolumn{1}{c|}{$\addf{\adds{\Tninfty}}$}&
31\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\Cref{-FMP+ES+OS=>CMMF}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tthree$}&
\multicolumn{1}{c|}{$\Tseven$}&\multicolumn{1}{c|}{$\addf{\Tthree}$}&
32\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\addnc{\Tbb}$}&\multicolumn{1}{c|}{$\addnc{\adds{\Tbb}}$}&
33\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\addnc{\Tbbinfty}$}&
34\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{2}{c|}{\cellcolor{red!15}}&
\multicolumn{1}{c|}{$\addnc{\Tninfty}$}&\multicolumn{1}{c|}{$\addnc{\adds{\Tninfty}}$}&
35\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|--}*{1}{>{\arrayrulecolor{black}}|-}--}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{2}{c|}{\multirow{-4}{*}{\cite{CADE}\cellcolor{red!15}}}&
\multicolumn{1}{c|}{$\Teight$}&\multicolumn{1}{c|}{$\addnc{\Tthree}$}&
36\\\hhline{-------------}

\multirow{7}{*}{$F$ } & \multirow{7}{*}{$F$ } &
\multirow{7}{*}{$T$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{$\Tleqone$}&\multicolumn{1}{c|}{$\adds{\Tleqone}$}&
\multicolumn{1}{c|}{$\addf{\Tleqone}$}&\multicolumn{1}{c|}{$\addf{\adds{\Tleqone}}$}&
37\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\Cref{-SI+ES=>CMMF}\cellcolor{red!15}}&\multicolumn{3}{c|}{\textcolor{red}{Unicorns 2.0}}&
38\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{2}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{$\Tleqn$}&\multicolumn{1}{c|}{$\adds{\Tleqn}$}&
\multicolumn{1}{c|}{$\addf{\Tleqn}$}&\multicolumn{1}{c|}{$\addf{\adds{\Tleqn}}$}&
39\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\Cref{-SI+ES=>CMMF}\cellcolor{red!15}}&\multicolumn{3}{c|}{\textcolor{red}{Unicorns 2.0}}&
40\\\hhline{~~~----------}

 &  &
 & \multirow{3}{*}{$F$ } &
\multirow{3}{*}{$T$ } & \multirow{3}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Toneodd$}&
\multicolumn{1}{c|}{$\Toddneq$}&\multicolumn{1}{c|}{$\addf{\Toneodd}$}&
41\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{CADE}\cellcolor{red!15}}}&\multicolumn{1}{c|}{$\Televen$}&
\multicolumn{1}{c|}{$\Tfourteen$}&\multicolumn{1}{c|}{$\addf{\Televen}$}&
42\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Ttwothreethree$}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tnequpinfty$}&
43\\\hline

\multirow{13}{*}{$F$ } & \multirow{13}{*}{$F$ } & \multirow{5}{*}{$T$ }
 & \multirow{5}{*}{$F$ } & \multirow{1}{*}{$T$ }
 & \multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ }
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tthreetwo$}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tthirteen$}&
44\\\hhline{~~~~---------}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{4}{*}{$T$ } &
\multirow{2}{*}{$T$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{$\Tmn$}&\multicolumn{1}{c|}{$\adds{\Tmn}$}&
\multicolumn{1}{c|}{$\addf{\Tmn}$}&\multicolumn{1}{c|}{$\addf{\adds{\Tmn}}$}&
45\\\hhline{~~~~~~~------}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\Cref{-SI+ES=>CMMF}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tten$}&
\multicolumn{1}{c|}{$\Ttwelve$}&\multicolumn{1}{c|}{$\addf{\Tten}$}&
46\\\hhline{~~~~~~-------}

 &  &
 &  &
 &  &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tmninfty$}&
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\addf{\Tmninfty}$}&
47\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}-}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{$\Tsix$}&
\multicolumn{1}{c|}{\multirow{-2}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{$\addf{\Tsix}$}&
48\\\hhline{~~-----------}

 &  &
\multirow{8}{*}{$F$ } & \multirow{8}{*}{$F$ } &
\multirow{4}{*}{$T$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tonebb$}&
\multicolumn{1}{c|}{$\Tbboneneq$}&\multicolumn{1}{c|}{$\addf{\Tonebb}$}&
49\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tbbinftythree$}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tbbneqinfty$}&
50\\\hhline{~~~~~---*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Toneinfty$}&
\multicolumn{1}{c|}{$\Toneinftyneq$}&\multicolumn{1}{c|}{$\addf{\Toneinfty}$}&
51\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tthreeone$}&
\multicolumn{1}{c|}{$\Tnine$}&\multicolumn{1}{c|}{$\adds{\Tnine}$}&
52\\\hhline{~~~~----*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
\multirow{4}{*}{$F$ } & \multirow{2}{*}{$T$ } &
\multirow{1}{*}{$T$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tnbb$}&
\multicolumn{1}{c|}{$\Tbbneq$}&\multicolumn{1}{c|}{$\addf{\Tnbb}$}&
53\\\hhline{~~~~~~--*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
\multirow{1}{*}{$F$ } & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Tmnbb$}&
\multicolumn{1}{c|}{\cite{FroCoS}\cellcolor{red!15}}&\multicolumn{1}{c|}{$\addf{\Tmnbb}$}&
54\\\hhline{~~~~~---*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 & \multirow{2}{*}{$F$ } &
\multirow{2}{*}{$F$ } & \multirow{1}{*}{$T$ } &
\multicolumn{1}{c|}{\cellcolor{red!15}}&\multicolumn{1}{c|}{$\Ttwoinfty$}&
\multicolumn{1}{c|}{$\Ttwoinftyneq$}&\multicolumn{1}{c|}{$\addf{\Ttwoinfty}$}&
55\\\hhline{~~~~~~~-*{1}{>{\arrayrulecolor{red!15}}|-}*{1}{>{\arrayrulecolor{black}}|-}---}

 &  &
 &  &
 &  &
 & \multirow{1}{*}{$F$ } &
\multicolumn{1}{c|}{\multirow{-8}{*}{\cite{FroCoS}\cellcolor{red!15}}}&\multicolumn{1}{c|}{$\Tfive$}&
\multicolumn{1}{c|}{$\Tfour$}&\multicolumn{1}{c|}{$\addf{\Tfive}$}&
56\\\hhline{-------------}
%\end{tabular}
%\vspace{-1em}
\caption[Caption for LOF]{Summarizing table.}
\label{tab-summary-app}
\end{longtable}

\renewcommand{\arraystretch}{1}}
